Combined subleading high-energy logarithms and NLO accuracy for W production in association with multiple jets

Large logarithmic corrections in $\hat s/p_t^2$ lead to substantial variations in the perturbative predictions for inclusive $W$-plus-dijet processes at the Large Hadron Collider. This instability can be cured by summing the leading-logarithmic contributions in $\hat s/p_t^2$ to all orders in $\alpha_s$. As expected though, leading logarithmic accuracy is insufficient to guarantee a suitable description in regions of phase space away from the high energy limit. We present (i) the first calculation of all partonic channels contributing at next-to-leading logarithmic order in $W$-boson production in association with at least two jets, and (ii) bin-by-bin matching to next-to-leading fixed-order accuracy. This new perturbative input is implemented in \emph{High Energy Jets}, and systematically improves the description of available experimental data in regions of phase space which are formally subleading with respect to $\hat s/p_t^2$.

==> Appendices/ExtremalQQbar.tex <==
% \subsection{Derivation of the Extremal $Q \bar{Q}$ Current}
% % \subsection{Derivation}
% \label{appendix:qqbar}

\begin{figure}[t]
\centering
\includegraphics[width=0.3\textwidth]{{qqbarex_schem}}
\caption{Schematic structure of the $gq \to \bar{Q}Qq$ amplitude in the limit
  $y_1 \sim y_2 \ll y_3$ which reduces to an effective $g \to \bar{Q} Q  g^*$
  vertex and a standard \HEJ current.}
\label{fig:qgimp}
\end{figure}

% We now derive the current for the production of an extremal quark-antiquark pair in rapidity
% from the process $g(p_a) q(p_b)  \rightarrow \bar{Q}(p_1) Q(p_2) q(p_3)$.
% We will take the limit where $y_1 \sim y_2 \ll y_3$, and hence
% we seek a result of the following form:
% \begin{align}
% iA_{gq \to \bar{Q}Qq} =g_s^3 T^d_{3b} \frac{  j^\mu_{q\bar{q}}(p_a, p_1, p_2) j_{\mu}(p_b,p_3) }{t_{b3}}.
% \label{eqn:NLLeqn}
% \end{align}

% \begin{figure}[btp]
% \centering
% \begin{subfigure}{0.45\textwidth}
% \centering
% \includegraphics{qqbarex1}
% \end{subfigure}
% \begin{subfigure}{0.45\textwidth}
% \centering
% \includegraphics{qqbarex2}
% \end{subfigure}
% \begin{subfigure}{0.45\textwidth}
% \centering
% \includegraphics{qqbarex4}
% \end{subfigure}
% \begin{subfigure}{0.45\textwidth}
% \centering
% \includegraphics{qqbarex5}
% \end{subfigure}
% \begin{subfigure}{0.45\textwidth}
% \centering
% \includegraphics{qqbarex3}
% \end{subfigure}
% \caption{The five tree-level graphs which contribute to the process $gq \to \bar{Q}Qq$.}
% \label{fig:qg_qQQ_graphs}
% \end{figure}

% There are five contributing diagrams at LO which are shown in
% \cref{fig:qg_qQQ_graphs}. By inspection we can see immediately
% that the diagrams in the second and third rows will be required as they contain
% the desired $t$-channel pole. However, we nevertheless include contributions from
% the first two diagrams as this allows us to preserve gauge invariance in all of phase space.
% These two diagrams give respectively:
% \begin{align}
% iA_s &= \phantom{-}\frac{i g_s^3 T^g_{3i} T^c_{ib} T^g_{21} }{s_{ab}s_{12}} \left[ \matel{3}{\mu}{a}2 p_b^\nu + \matel{3}{\nu}{a} \matel{a}{\mu}{b} \right] \matel{2}{\mu}{1} \varepsilon_\nu (p_a),\label{eq:schanqqex}\\
% iA_u &= -\frac{i g_s^3 T^c_{3i} T^g_{ib} T^g_{21} }{s_{a3}s_{12}} \left[ \matel{3}{\mu}{b}2 p_3^\nu - \matel{3}{\nu}{a} \matel{a}{\mu}{b}\right] \matel{2}{\mu}{1} \varepsilon_\nu (p_a	).\label{eq:uchanqqex}
% \end{align}
% Examining the two terms in brackets in \cref{eq:schanqqex}, the first term will have a
% magnitude like $\sqrt{s_{23} s_{b1}}$ or $\sqrt{s_{13} s_{b2}}$ after contraction with the current $\matel{2}{\mu}{3}$ (depending on the choice of helicities), whereas the second term will have a
% magnitude which goes like $\sqrt{s_{a2} s_{b1}}$ or $\sqrt{s_{a1} s_{b2}}$. Thus in the limit $y_1 \sim y_2 \ll y_3$, the second term is suppressed relative to the first.
% Neglecting this term we obtain:
% \begin{align}
% \label{eq:labelAs}
% iA_s \approx \frac{i g_s^3 T^g_{3i}T^c_{ib}T^g_{21}}{s_{ab}s_{12}} 2p_b^\nu \matel{3}{\mu}{b} \matel{2}{\mu}{1} \varepsilon_\nu (p_a).
% \end{align}
% Applying similar argments to \cref{eq:uchanqqex} yields:
% \begin{align}
% \label{eq:labelAu}
% iA_u \approx \frac{-i g_s^3 T^c_{3i}T^g_{ib}T^g_{21}}{s_{a3}s_{12}} 2p_3^\nu \matel{3}{\mu}{b} \matel{2}{\mu}{1} \varepsilon_\nu (p_a).
% \end{align}
% Although both of these terms now contain the desired current $j_{\mu}(p_b,p_3) =
% \matel{3}{\mu}{b}$ they do not yet have the expected colour
% structure. However, in the high energy limit we have $p_b \sim p_3$.
% Upon applying this limit \cref{eq:labelAs,eq:labelAu} become identical up to a
% relative minus sign.  The colour algebra gives
% \begin{align}
%   (T^g_{3i}T^c_{ib}- T^c_{3i}T^g_{ib}) = i f^{gcd}T^d_{3b},
% \end{align}
% which leads to
% \begin{align}
%   \label{eq:A1plusA2}
%   i(A_s + A_u) \approx g_s^3 T^d_{3b}\frac{j_{\mu}(p_b,p_3)}{t_{b3}}\left(-f^{gcd}T^g_{21}\frac{2p_b^\nu q_2^2 \matel{2}{\mu}{1} \varepsilon_\nu (p_a)}{s_{ab}s_{12}}\right),
% \end{align}
% where $q_2^2 = (p_a-p_1-p_2)^2$.

% No approximation is required for the remaining three diagrams, and summing the
% full expressions together with \cref{eq:A1plusA2} gives
% \begin{equation}
% \label{eq:Qfinal}
%  j^\mu_{q\bar{q}}(p_a, p_1, p_2) = -i \varepsilon_\nu(p_a) \left[ T^d_{2i}T^c_{i1}(U^{\mu\nu}_{1,q\bar{q}} + L^{\mu\nu}_{q\bar{q}}) - T^c_{2i}T^d_{i1} (U^{\mu\nu}_{2,q\bar{q}} + L^{\mu\nu}_{q\bar{q}} ) \right]
% \end{equation}
% where
% \begin{align}
%  U^{\mu\nu}_{1,q\bar{q}} &= \frac{1}{t_{a1}} \left( 2p_1^\nu \matel{2}{\mu}{1} - \matel{2}{\mu}{a}\matel{a}{\nu}{1} \right) \\
%  U^{\mu\nu}_{2,q\bar{q}} &= \frac{1}{t_{a2}} \left( 2p_2^\nu \matel{2}{\mu}{1} - \matel{2}{\nu}{a}\matel{a}{\mu}{1} \right) \\
%  L^{\mu\nu}_{q\bar{q}} &=  \frac{1}{s_{12}} \left(\frac{2 p_b^\nu q_2^2}{s_{ab}} \matel{2}{\mu}{1}
%  + \left(2(p_1 + p_2)^\nu \eta^{\mu\rho} - 2p_a^\mu \eta^{\rho \nu} + 2p_a^\rho \eta^{ \nu \mu}\right) \matel{2}{\rho}{1} \right)
% \end{align}

% %
% %
% % \begin{align}
% % \label{eq:Qfinal}
% % \begin{split}
% % j^\mu_{q\bar{q}} = \varepsilon_\nu(p_b) &\left[
% %  -i\frac{C_1}{t_{b3}} \left(\bar{u}_2 \gamma^\mu (\slashed{p}_3-\slashed{p}_b) \gamma^\nu v_3 \right)
% % + i\frac{C_2}{t_{b2}} \left( \bar{u}_2 \gamma^\nu (\slashed{p}_2-\slashed{p}_b)\gamma^\mu v_3 \right) \right. \\
% % & \left.\:\: -\frac{C_t}{s_{23}} \left(\frac{2 p_a^\nu q_1^2}{s_{ab}}
% % \matel{2}{\mu}{3} + V^{\mu \rho \nu}_{3g}
% % \matel{2}{\rho}{3} \right) \right],
% % \end{split}
% % \end{align}
% % where
% % \begin{align}
% % V_{3g}^{\mu \rho \nu} &=(2p_2 + 2p_3)^\nu \eta^{\mu\rho} - 2p_b^\mu \eta^{\rho \nu} + 2p_b^\rho \eta^{ \nu \mu},
% % \end{align}
% % and the colour factors are given by
% % \begin{align}
% %   \label{eq:Cextremal}
% %     C_1 = T^d_{2i}T^b_{i3}, \qquad C_2 = T^b_{2i}T^d_{i3},
% %   \quad {\rm and} \quad C_t = f^{gbd}T^g_{23}.
% % \end{align}
% % We note that these are not all independent, and we can choose to make the
% % replacement $iC_t=C_1-C_2$, which yields a very similar form to that for the
% % unordered gluon current in Eq.~\eqref{eq:unoderiv}.

% The full leading-order
% calculation must be gauge-invariant, but we must check that this still holds
% after the approximations made above. As in the analogous case of unordered
% emissions, one may readily demonstrate that
% \begin{equation}
%  p_{a\nu}L^{\mu\nu}_{q\bar{q}} = -p_{a\nu} U^{\mu\nu}_{1,q\bar{q}} = -p_{a\nu}U^{\mu\nu}_{2,q\bar{q}}
% \end{equation}
% everywhere in phase space and thus \cref{eq:Qfinal} satisfies the appropriate Ward identity.

% We can now define :
% \begin{equation}
% \label{eq:current_qqbar}
%  \left|\mathcal{J}_{gQ\to \bar{q}qQ}\right|^2 = \frac{ (g_s^2)^3 C_F^2}{4(\Nc^2-1)} \left\|S_{gQ\to \bar{q}qQ}\right\|^2
% \end{equation}
% where
% \begin{align}
%   \label{eq:Sunoext}
%   \begin{split}
%     \left\|S_{gQ\to \bar{q}qQ}\right\|^2 &= \sum_{h_a,h_1,h_b,h_n}\ \bigg[
%     2\mathrm{Re}\big( [(L^{\mu\nu}+U^{\mu\nu}_{1,q\bar{q}})\cdot j_{nb\, \mu}]\ [
%           (L^{\rho}_{\;\,\nu}+U_{2\;\, \nu}^{\;\rho})\cdot j_{nb\, \rho} ]^* \big) \\
%     & \hspace{4cm} - 2\frac{C_F}{C_A} \left| (U_1^{\mu\nu}+U_2^{\mu\nu}) \cdot
%         j_{nb_\mu} \right|^2 \bigg].
%   \end{split}
% \end{align}

